A Comparative Analysis Between the Additive and the Multiplicative Extended Kalman Filter for Satellite Attitude Determination

The general consensus is that the Multiplicative Extended Kalman Filter (MEKF) is superior to the Additive Extended Kalman Filter (AEKF) based on a wealth of theoretical evidence. This paper deals with a practical comparison between the two filters in simulation with the goal of verifying if the previous theoretical foundations are true. The AEKF and MEKF are two variants of the Extended Kalman Filter that differ in their approach to linearizing the system dynamics. The AEKF uses an additive correction term to update the state estimate, while the MEKF uses a multiplicative correction term. The two also differ in the state of which they use. The AEKF uses the quaternion as its state while the MEKF uses the Gibbs vector as its state. The results show that the MEKF consistently outperforms the AEKF in terms of estimation accuracy with lower uncertainty. The AEKF is more computationally efficient, but the difference is so low that it is almost negligible and it has no effect on a real-time application. Overall, the results suggest that the MEKF is a better choise for satellite attitude estimation due to its superior estimation accuracy and lower uncertainty, which agrees with the statements from previous work

==> Content/09_Useful.tex <==
\subsection{Triaxial Attitude Determination}
Another method for determining the attitude of a satellite given two unit vectors in two different frames is the TRIaxial Attitude Determination (TRIAD) algorithm.
Similar to the Wabha problem, here there are two sets of observations, one in the body frame, \textbf{b}, and one in the reference frame, \textbf{r},
and the goal is to find the attitude matrix \textbf{A} that takes the reference observation to the body frame observation, $\textbf{Ar} = \textbf{b}$

The two unit vectors are from two different star trackers. Due note that there is a difference factor of $2\cdot 10^10$ between the furthest satellite and the closest star which means that the translational locations of the body frame of the satellite and the Earth are approximately the same and thus only the rotations has to be estimated.

\begin{figure}[htbp]
    \centering
    \includegraphics[width = 0.2\textwidth]{Images/TRIADAlgorithm.png}
    \caption{Caption}
    \label{fig:TRIAD}
\end{figure}

Consider the direction of two stars that are known with respect to the Earth’s reference frame. These directions are denoted by the vectors $X_{r1}$ and $X_{r2}$ as seen in \ref{fig:TRIAD}. The stars are identified on the star trackers which are placed orthogonally to each other to make sure the system is over determined. From these two star trackers the star vectors of $X_{b1}$ and $X_{b2}$ are observed.
Two orthonormal bases can be made from the two sets of observations. The first vector, which is usually the most precise observation, is chosen as the first column of the basis. The cross product between the two observations is made to make an orthogonal vector to the first. The last column of the basis is given by taking the cross product of the two found vectors.
A basis for the reference frame looks like this

\begin{equation}\label{eq:basisforref}
    v_1=r_1,v_2=\frac{r_1 \times r_2}{\left\| r_1 \times r_2\right\|},v_3=r_1 \times v_2
\end{equation}

and the same is true for the body frame by substituting $v$ with $w$ and $r$ with $b$.
And, remembering the problem $\textbf{Ar} = \textbf{b}$, it can be substituted with \ref{eq:basisforref}

\begin{gather}
    \textbf{A}[v_1v_2v_3] = [w_1w_2w_3]\\\nonumber
    \textbf{A} = [w_1w_2w_3][v_1v_2v_3]^T
\end{gather}

And so the attitude matrix can be determined from two unit vectors.


The same way that a star is projected onto the image of a star tracker, the mathematics to artificially project an emulated star onto a field can be done by perceiving the star tracker as an ideal pin hole camera with a focal length \textit{f}.
A certain star that is known a priori, e.g. from a star database is detected with a certain point $P$ in $[X_i, Y_i, Z_i]$ where $i$ denotes that it is in the inertial frame of the Earth.
The attitude of the satellite is given by the axis $[R_x, R_y, R_z]$ which is the quantity that is ought to be estimated. However, as there is a need to emulate the sensor, the attitude is used to project the point P onto the image plane as can be seen in \ref{fig:projection}

\begin{figure}[htbp]
\centerline{\includegraphics[width = 0.2\textwidth]{Images/projection.png}}
\caption{A star being projected on the image plane}
\label{fig:projection}
\end{figure}

The $Z_i$ in the point $P$ has to be expressed in the body frame, which can be done by projecting onto $R_z$

\begin{equation}
    Z_b = <R_z, P>
\end{equation}

Where $<>$ denotes the inner product between the two.
From \ref{fig:projection}, a similarity triangle can be observed from which useful factors can be deduced. The point of intersection between the image plane and the star projection is the point $x'$ and thus the actual location of the star can be deduced from the projection

\begin{equation}\label{eq:similartriangles}
    \frac{x'}{f} = \frac{<R_x,P>}{<R_z,P>} \Leftrightarrow x' = f\frac{<R_x,P>}{<R_z,P>}
\end{equation}

The same convention holds true for $y'$ by substituting $R_x$ with $R_y$ in \ref{eq:similartriangles}

The star vector can be expressed in the body frame of the satellite as such

\begin{equation}
    S=\frac{1}{\sqrt{f^2+x'^2+y'^2}}
    \begin{bmatrix}
    x'\\
    y'\\
    f
\end{bmatrix}
\end{equation}



Equation \ref{eq:Wahba} can be simplified by expanding $||\textbf{b}_i - \textbf{Ar}_i||^2$ using the fact that \textbf{b} and \textbf{r} will have the norm $1$ and remembering that the trace is $tr(u_1u_2^T) = u_1^Tu_2 = u_1\bullet u_2$

\begin{equation}
    ||\textbf{b}_i-\textbf{Ar}_i||^2 = ||\textbf{b}_i||^2+||\textbf{Ar}_i||^2 - 2\textbf{b}_i\bullet \textbf{Ar}_i = 2-2tr(\textbf{Ar}_i\textbf{b}_i^T)
\end{equation}

The larger $tr(\textbf{Ar}_i\textbf{b}_i^T)$, the more the original cost function is minimized \cite{b9}. The cyclic property of the trace operator can be used to further simplify the cost function into the attitude profile matrix \textbf{B}, and the cost function can be converted into \ref{eq:WahbaNewCost}

\begin{equation}\label{eq:WahbaNewCost}
    \operatorname*{arg\space max}_{ \left\| \textbf{A}\right\| =1}=tr(\textbf{AB}^T)
\end{equation}

And after performing the algebraic steps as described in \cite{b10}, the Davenport matrix \textbf{K} can be introduced as

\begin{equation}
    \textbf{K} = \begin{bmatrix}
     tr(\textbf{B})    & \textbf{z}^T\\
      \textbf{z} & \textbf{S}-I\cdot tr(\textbf{B})
    \end{bmatrix}
\end{equation}

Where 

\begin{equation}
    \textbf{S} = \textbf{B}+\textbf{B}^T
    \textnormal{ and }
    \textbf{z} = \begin{bmatrix}
        \textbf{B}_{23}-\textbf{B}_{32}\\
        \textbf{B}_{31}-\textbf{B}_{13}\\
        \textbf{B}_{12}-\textbf{B}_{21}
    \end{bmatrix} =
    \sum_{i=0}^na_i(\textbf{b}_i\times\textbf{r}_i)
\end{equation}


and has the following relation
\begin{equation}
    tr(\textbf{AB}^T)=\textbf{q}^T\textbf{Kq}
\end{equation}

\begin{equation}\label{eq:WahbaFinalCost}
    \bold{A}=\operatorname*{arg\space max}_{ \left\| \textbf{A}\right\| =1}=tr(\textbf{AB}^T)=\textbf{q}^TK\textbf{q}
\end{equation}

As mentioned, the quaternion has the norm constraint $1$ and the lagrangian for the optimization problem can be introduced as
\begin{equation}
\label{eq:langrangian}
    L(A(\textbf{q}),\lambda)=\lambda(\textbf{q}^T\textbf{q}-1)-\textbf{q}^TK\textbf{q}
\end{equation}
The extrema of the Lagrangian happens when the derivative of the Lagrangian is zero and thus this can be simplified into 

Unused cites:
\bibitem{b9} Yaakov Oshman and Avishy Carmi. “Attitude Estimation from Vector Observations Using a Genetic-Algorithm-Embedded Quaternion Particle Filter”. In: Journal of Guidance Control and Dynamics - J GUID CONTROL DYNAM 29 (July 2006), pp. 879–891. do i: 10.2514/1.17951.

\bibitem{b10} Jason (https://math.stackexchange.com/users/290434/jason). Davenports Q-method (Finding an orientation matching a set of point samples). Mathematics Stack Exchange. URL:https://math.stackexchange.com/q/1634113

\bibitem{b11} Zamani, et. al. (2015). Nonlinear Attitude Filtering: A Comparison Study. 


POSTER!!!!


% Introduction
Satellite determination is the process of determining the location and orientation of a satellite in space. In this paper, the focus is on the Additive Extended Kalman Filter (AEKF) and the Multiplicative Extended Kalman Filter (MEKF) 

There are different thoughts about the two derivatives of the Kalman filter and which is best. From [6] it is noted that numerical issues surrounding AEKF might arise, but this caused no issues in a practical application. In [12] it was concluded that using brute force normalization, the AEKF was optimal under standard non-linear filtering assumptions, and that the MEKF is not superior to the AEKF.
In [3], it is concluded that there is not valid reason for using the AEKF over the MEKF due to the lower computational time and stronger foundation

The aim of this paper is to implement and compare the two filters side by side

It is therefore the aim of this paper is to implement the two filters and compare them side by side while determining the attitude of a satellite with sensors such as a gyroscope and a star tracker.


% Methods
% Quaternion representation
% Star tracker outputs a quaternion
% Davenport*
% AEKF and MEKF

The quaternion is the representation with the lowest-dimensionality free of gimbal lock. It is composed of a scalar and a vector part, where the scaler represents the amount of rotation around the vector.

Equation

It must obey the normalizing constraint to remain a valid representation

Equation

The Gibbs vector is useful for representing the orientation of objects in three-dimensional space, as the orientation can be represented by the direction of the Gibbs vector. I can be extracted from a quaternion as such

Equation
|
The kinematic equation of the quaternion describes how it changes over time and is given by

The Kalman Filter uses a model of the system and measurement data to provide accurate estimates of the state of the system over time.
Its derivatives, the AEKF and MEFK differ in the way they handle errors. The AEKF adds the error to the measured data while the MEKF multiplies it.


The AEKF follows the standard update equations as the EKF, but the MEKF finds the correct quaternion from the quaternion product between the estimate and the error quaternion.
% Results




% Discussion
Two different derivations of the KF, specifically the AEKF and the MEKF have been implemented in simulation with the goal of comparing the two to evaluate if the MEKF is so superior as stated in previous work. Each filter uses the quaternion representation, where the norm is constrained to $1$. Each instance of the filters uses measurements obtained from multiple emulated star trackers, where the Davenport q-method algorithm has been employed to determine the attitude of the satellite. The key difference between the two filters is in the way the error is obtained. As the names may suggest, the error quaternion is obtained through addition in AEKF and through the quaternion multiplication in MEKF.
The results from the study shows that the MEKF is more stable than the AEKF in terms of the norm of the absolute error. It was also seen how the lower dimensionality caused the MEKF to have a lower computational time than the AEKF. The conditioning number of the MEKF was considerably larger than the AEKF which was not expected as the literature stated that the AEKF would have had higher conditioning number. 
The aim of the paper was to compare the Additive and the Multiplicative Extended Kalman Filter in a more practical sense than in the related works. To this end, implementations were simulated with multiple star trackers and a gyroscope as measurements to determine the attitude of a satellite.
The results were expected and showed the MEKF with a smaller absolute error than the AEKF and was more stable in its estimation. The comparison between the covariance matrices showed that the covariance matrix of the MEKF had more certainty  than the AEKF. The MEKF was better in terms of computation time however did have a larger conditioning number in the covariance matrix. 
Despite this, the MEKF had in general much better stability and was more resilient to noisy measurements.
The paper can conclude that based on the lower dimensionality, error, computational time, uncertainty, and lower variance of the error, the MEKF is better than the AEKF in the context of satellite attitude determination, which supports current opinion in the satellite attitude community.


The aim of the paper was to compare the AEKF and the MEKF in a more practical sense than in the related works. To this end, implementations were simulated with multiple star trackers and a gyroscope as measurements to determine the attitude of a satellite.
The results were expected and showed the MEKF with a smaller absolute error than the AEKF and was more stable in its estimation. The comparison between the covariance matrices showed that the matrix for MEKF was smaller and thus more certain in the estimated state than the AEKF.
The conditioning number of both the MEKF and the AEKF were approximately equal around $1$, which differs from the literature, where it was stated that the AEKF would have a higher conditioning number. A large conditioning number indicates that the matrix being inverted is poorly conditioned, meaning that it is close to being singular or degenerate. In this case, neither filter were close to being singular.
Overall, the MEKF had much better stability and was more resilient to noisy measurements.
One reason for the superior performance of the MEKF is that it is able to better capture the nonlinearities present in many systems. The AEKF assumes that the process and measurement noise are additive, which can lead to errors when dealing with nonlinear systems. In contrast, the MEKF uses a multiplicative noise model, which allows it to more accurately estimate the state of nonlinear systems, which is in line with the consensus from the literature.
% Refs

